CoMeFa: Compute-in-Memory Blocks for FPGAs

Block RAMs (BRAMs) are the storage houses of FPGAs, providing extensive on-chip memory bandwidth to the compute units implemented using Logic Blocks (LBs) and Digital Signal Processing (DSP) slices. We propose modifying BRAMs to convert them to CoMeFa (Compute-In-Memory Blocks for FPGAs) RAMs. These RAMs provide highly-parallel compute-in-memory by combining computation and storage capabilities in one block. CoMeFa RAMs utilize the true dual port nature of FPGA BRAMs and contain multiple programmable single-bit bit-serial processing elements. CoMeFa RAMs can be used to compute in any precision, which is extremely important for evolving applications like Deep Learning. Adding CoMeFa RAMs to FPGAs significantly increases their compute density. We explore and propose two architectures of these RAMs: CoMeFa-D (optimized for delay) and CoMeFa-A (optimized for area). Compared to existing proposals, CoMeFa RAMs do not require changing the underlying SRAM technology like simultaneously activating multiple rows on the same port, and are practical to implement. CoMeFa RAMs are versatile blocks that find applications in numerous diverse parallel applications like Deep Learning, signal processing, databases, etc. By augmenting an Intel Arria-10-like FPGA with CoMeFa-D (CoMeFa-A) RAMs at the cost of 3.8% (1.2%) area, and with algorithmic improvements and efficient mapping, we observe a geomean speedup of 2.5x (1.8x), across several representative benchmarks. Replacing all or some BRAMs with CoMeFa RAMs in FPGAs can make them better accelerators of modern compute-intensive workloads.

==> 06_discussion.tex <==
\section{Discussion} \label{section:discussion}


\subsection{Benefits}
The following describe the advantages of using \wnameRAMs~qualitatively.
\begin{enumerate}
    \item \wnameRAMs~transform BRAMs, which can only be used for storage, into highly parallel SIMD engines. This parallelism provides significant throughput boost for an FPGA. 
    %Applications can be sped up and execute in shorter time compared to a normal FPGA. 
    When not computing, \wnameRAMs~can still function as normal BRAMs (data does not need to be transposed).
    
    \item Because the computation happens inside the memory block, data movement between various blocks on the FPGA is significantly reduced. 
    The requirement of precious routing/interconnect resources is reduced. This leads to reduction in power consumption, reduced routing congestion, and potentially faster frequencies.
    
    \item Any custom operation with any custom precision can be supported by a \wnameRAM~block.  
    %For performing a different operation or for using a different precision, a different instruction sequence needs to be generated and applied to the \wnameRAM. 
    This makes \wnameRAMs~universally applicable for any application domain.
    %There is no hardened logic to support for specific operations or specific precisions, making \wnameRAMs~very flexible like a Logic Block.
    
    \item \wnameRAMs~increase the effective bandwidth available for computation. In one block, 160 data bits can be processed in parallel, instead of 40 (maximum data port width of a BRAM; an external block like DSP/LB can only access 40 bits from a BRAM at a time). 
    %A user needing wide shallow BRAMs, that provide high bandwidth but utilize BRAMs poorly, can use a \wnameRAM~with higher utilization instead. 
    
    \item Replacing BRAMs in an FPGA with \wnameRAMs~increases the compute density of FPGAs ($GOPS/mm^2$). A smaller Silicon area will potentially be required for a given circuit. And this means that larger circuits can fit on the same FPGA.  
\end{enumerate}

%Can be shrinked into a table or integrated into the benefits section, by adding a pointer for variable application support at its end and just adding the list given in this section in short. (Basically integrate it with benefits subsection)

\subsection{Applications and Usage}
\wnameRAMs~are universal blocks and can be used for accelerating any application. In some ways, \wnameRAMs~can be thought of blocks that fuse together Logic Blocks and BRAMs. They provide a more structured way of computation compared to Logic Blocks, along with storage capability of BRAMs. They are more flexible  than DSP Slices owing to their precision agnosticism. However, they take longer for one operation compared to a DSP Slice (if the DSP Slice supports that kind of operation) because of their bit-serial nature, although in most cases, this latency can be hidden or overlapped with other operations. The parallelism \wnameRAMs~provide (SIMD) is different than the pipeline parallelism that is commonly used with Logic Blocks and DSP Slices. Data parallelism (split the data to be processed between traditional DSP and LB based compute units, and  \wnameRAM~based compute units) can be used as well. Some applications that are better suited for deploying \wnameRAMs~than others are:
\begin{enumerate}
    \item Applications which have significant inherent parallelism. E.g. image processing and deep learning.
    \item Applications that do not require a lot of communication between processing elements. E.g. elementwise and bitwise operations.
    \item Applications that use reduced and/or custom numerical precisions. E.g. deep learning.
    \item Applications that can tolerate high latency, in lieu of high throughput. E.g. video encoding/compression in non-real time applications.
\end{enumerate}

%\wnameRAMs~are not replacements of DSPs or LBs, but can work together and complement them. 
%One way of achieving speedup using \wnameRAMs~is to split the data to be processed between traditional DSP and LB based compute units (which are fed by BRAMs), and  \wnameRAM~based compute units (which store as well as process data). Let's consider the case where, time $T$ was spent on processing $D$ chunks of data on a baseline system (using only traditional compute units). However, if a part of the data (e.g. $D/3$ chunks) is processed by \wnameRAMs~and if the rest of the data ($2D/3$) is processed by traditional compute units in parallel, then the total time taken would be less than $T$ (say $2T/3$). This achieved speedup depends on the distribution of work between traditional units and \wnameRAM~based units, and the best case would be when both type of units finish in approximately equal amount of time. 


\subsection{Comparison with Related Work}

The most relevant related works are Computational RAMs \cite{computational_ram} and Compute Capable BRAMs \cite{ccb}. Table \ref{table:diff_ccb_comefa} shows the differences between C-RAM, CCB and \wname.

\begin{comment}



\subsection{Computational RAM}
In Computational RAM (or C-RAM) \cite{computational_ram}, a row of processing elements (PEs) is added to a DRAM or SRAM. Each PE is pitch-matched with a memory column. Two PE architectures were proposed - A simpler PE supporting bit-serial computation and a more complex PE with bit-parallel support. Our proposal, \wnameRAMs, is influenced by C-RAMs, but there are many differences. \wnameRAMs~are targeted specifically for FPGAs. In C-RAM, operations take 3 cycles - one cycle to read the first operand row, second cycle to read the second operand row and a third cycle to compute and write the result back. This avoids changing the sequencing logic inside the RAM to generate events for read/write operation (wordline activation, precharge, sense amp enable, etc), but requires additional flip-flops to store the operands in the PE increasing its area.  \wnameRAMs, on the other hand, take only 1 (although longer) cycle to perform an operation, do not require flip-flops to store operands across cycles, and modify the sequencing logic inside the RAM. Also, \wnameRAMs~do not have a bus for PE to PE communication, like in C-RAMs.



\subsection{Compute Capable BRAMs}

%\wnameRAMs~are similar to Compute Capable RAMs (CCB) in that they use bit-serial compute, add processing elements near the sense amplifiers, and use a transposed data layout. 
Compute Capable RAMs (CCB) are targeted for FPGAs and specifically for DL applications.
\wnameRAMs~have many differences with CCBs. \wnameRAMs~rely on the fact that FPGA BRAMs are already true dual ported, and use this feature to read two operand bits in 1 clock cycle. On the other hand, CCBs 
%change the underlying behavior of the SRAM array. That is, they 
activate two word-lines at the same area and the AND/NOR of two operand bits is read at the sense amplifiers. To avoid data corruption because of multi-row access, the wordline voltage has to be lowered significantly. This is required to ensure robustness and high margins. A separate voltage source is required to provide this reduced voltage. Reduction in voltage reduces the frequency significantly by 1.6x. An additional row decoder is also required for multi-row access. 
In \wnameRAMs, no changes to sense amplifiers are required on either port. In CCBs, one port's sense amplifiers are modified. One sense amplifier for each pair of bitlines (BL/BLB) is replaced with two sense amplifiers (one with BL/Vref and second with BLB/Vref). 
In addition, BRAMs employ column multiplexing. To read all bitline pairs at the same time, additional sense amplifiers are required to be added. So, there is area overhead as well as delay overhead in CCB. In \wname, we present two architectures - one delay-optimized and another area-optimized.
Additionally, the PEs in \wnameRAMs~are very flexible and can perform any 2-bit operation on the operands. Floating point operations are also supported. The PEs in CCB only support addition based operations for fixed-point precision. In CCB, there is no communication between various CCB blocks. \wnameRAMs~provide chaining between neighboring blocks allowing for communication between the PEs.
\end{comment}



TODO: Move table to Evaluation/Implementation section


 
 
 
 

==> acknowledgment.tex <==
%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
\begin{acks}
\noindent
%{\bf{Acknowledgement:}}
This research was supported in part by National Science Foundation (NSF) grant number 1763848. Any opinions, findings, conclusions or recommendations are those of the authors and not of the NSF.

\end{acks}


==> keywords.tex <==
%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{FPGA; neural networks; deep learning; hardware acceleration; computer architecture; processing in memory; sram; block rams}

